Testing Spacecraft Formation Flying with Crazyflie Drones as Satellite Surrogates

As the space domain becomes increasingly congested, autonomy is proposed as one approach to enable small numbers of human ground operators to manage large constellations of satellites and tackle more complex missions such as on-orbit or in-space servicing, assembly, and manufacturing. One of the biggest challenges in developing novel spacecraft autonomy is mechanisms to test and evaluate their performance. Testing spacecraft autonomy on-orbit can be high risk and prohibitively expensive. An alternative method is to test autonomy terrestrially using satellite surrogates such as attitude test beds on air bearings or drones for translational motion visualization. Against this background, this work develops an approach to evaluate autonomous spacecraft behavior using a surrogate platform, namely a micro-quadcopter drone developed by the Bitcraze team, the Crazyflie 2.1. The Crazyflie drones are increasingly becoming ubiquitous in flight testing labs because they are affordable, open source, readily available, and include expansion decks which allow for features such as positioning systems, distance and/or motion sensors, wireless charging, and AI capabilities. In this paper, models of Crazyflie drones are used to simulate the relative motion dynamics of spacecraft under linearized Clohessy-Wiltshire dynamics in elliptical natural motion trajectories, in pre-generated docking trajectories, and via trajectories output by neural network control systems.

==> Notes_Questions/CR_CWH_Background.tex <==
The linearized Clohessy-Wiltshire equations describing the motion of satellites are the equations implemented for testing in this paper. They take two forms, being discrete and continuous, but both take the same basic structure: 
\begin{equation}
{\bf \dot{x}} = {A \bf{x} + B \bf{u}}
\end{equation}
x is a vector describing current position and velocity of the satellite being examined, taking the form [X, Y, Z, Xdot, Ydot, Zdot], and u is a vector describing the control forces for the satellite taking the form [Fx, Fy, Fz]. For the continuous form, the A and B matrices are:
\[A =\ 
\begin{bmatrix}
    0 & 0 & 0 & 1 & 0 & 0\\
    0 & 0 & 0 & 0 & 1 & 0\\
    0 & 0 & 0 & 0 & 0 & 1\\
    3n^2 & 0 & 0 & 0 & 2n & 0\\
    0 & 0 & 0 & -2n & 0 & 0\\
    0 & 0 & -n^2 & 0 & 0 & 0\\
\end{bmatrix}\]
and,
\[B =\
\begin{bmatrix}
    0 & 0 & 0\\
    0 & 0 & 0\\
    0 & 0 & 0\\
    1/m & 0 & 0\\
    0 & 1/m & 0\\
    0 & 0 & 1/m\\
\end{bmatrix}\]
Wherein m is the mass of the satellite and n is its mean motion. \\In the discrete form, the A and B matrices are:
\[A =\
\begin{bmatrix}
    4-3*cos(n*t) & 0 & 0 & (1/n)*sin(n*t) & (2/n)*(1-cos(n*t)) & 0\\
    6*(sin(n*t)-n*t) & 1 & 0 & (-2/n)*(1-cos(n*t)) & (1/n)*(4*sin(n*t)-3*n*t) & 0\\
    0 & 0 & cos(n*t) & 0 & 0 & (1/n)*sin(n*t)\\
    3*n*sin(n*t) & 0 & 0 & cos(n*t) & 2*sin(n*t) & 0\\
    -6*n*(1-cos(n*t)) & 0 & 0 & -2*sin(n*t) & 4*cos(n*t)-3 & 0\\
    0 & 0 & -n*sin(n*t) & 0 & 0 & cos(n*t)\\
\end{bmatrix}\]
and,
\[B =\
\begin{bmatrix}
    (1/n)*(cos(n*t)-1) & (2/n)*(t+(1/n)*sin(n*t)) & 0\\
    (-2/n)*(t-(1/n)*sin(n*t)) & (1/n)*((-4/n)*(cos(n*t)-1)-(3*n/2)*t**2) & 0\\
    0 & 0 & (-1/n**2)*(cos(n*t)-1)\\
    (1/n)*sin(n*t) & (-2/n)*(cos(n*t)-1) & 0\\
    (2/n)*(cos(n*t)-1) & (4/n)*(sin(n*t)-3*t) & 0\\
    0 & 0 & (1/n)*sin(n*t)\\
\end{bmatrix}\]
Where again n is a value representing the mean motion of the satellite.

==> Notes_Questions/CR_ES.tex <==
\section{Experimental Setup}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Overview}
The simulated testing of satellite trajectories proceeds, in this implementation, as follows. First, the trajectory is calculated, then it is scaled down to an appropriate size to be flown on a crazyflie 2.x and fit into waypoints that the crazyflie can follow. Then a flight simulation is run wherein the desired waypoints are fed to the crazyflie, and the crazyflie's state is observed during this simulated flight for the use of a simple PID controller. This general structure is illustrated in the workflow block diagram in figure [].
￼

\subsection{Trajectory Creation}
There are multiple implementations to the creation of the satellite trajectory, all of which calculate the linearized hill's equations discussed in background of this paper.

%%% Amount of detail can be adjusted for more focus in this section or in the appendix %%%
The primary difference between these implementations is whether the equations are in their continuous or discrete expression. Both have fully implemented the A and B matrices which handle current state of and current control inputs of the satellite, respectively. The control inputs are set to be zero in x, y, and z for natural motion trajectories, but the inclusion of these control forces allows for the testing of controlled satellite trajectories, which is the natural progression of terrestrial satellite testing and is likely to be of much higher interest moving forward. 

%% One important similarity between the two implementations is the ability to adjust the orbital period of the trajectory independently from the adjustment of the runtime/trajectory creation. The significance of this similarity can best be understood with the explanation of waypoint creation. %%


\subsection{Waypoint Creation}
After the trajectory is made, it must be scaled for use with the crazyflies and then fit into waypoints to be communicated to the crazyflie. This can be understood by examining the communication between the crazyflie drone and any script it works with. As explained \hl{in the background}, this communication is done at a certain frequency through the use of the crazyradio, and for the control of the drone in simulation, this is done at a frequency of 48 Hz []. It is necessary for any trajectory to be fit into waypoints updated at this frequency for the trajectory to be communicated. This is where the major differences between continuous and discrete implementations arise. To be fit into the correct format for communication, the continuous implementation uses an iterative solver with an adjustable step size that fits the result into waypoints upon the calculation of the trajectory. The discrete implementation uses no solver, and its solution is formatted correctly by being solved iteratively with a constant step size. 

% However, extending the simulation runtime necessitates the number of waypoints to grow larger. This explains the significance of the ability to adjust the orbital period of the trajectory independently from the runtime of the simulation/trajectory creation.

% The number of iterations to be run through is calculated with the step size and the runtime, so the correct number of waypoints are always saved. which allows for intuitive time scaling that allows for the trajectory progression to be sped up or slowed down, as well as the total runtime to be extended or shortened. This is successfully implemented in both implementations.


\subsection{Simulation Flight}
\textcolor{red}{note - explain the PID controller in this section}
Now that the trajectories have been calculated, scaled, and formatted correctly, the remaining step is for this trajectory to be fed to the crazyflie and its flight following this trajectory is simulated. Within the scope of this paper, it is worth briefly detailing the observation and control of the crazyflie within the gym environment. For observation, an observation vector is made for each step of the gym environment including 16 pieces of information: position and velocity in x, y, and z, the quaternions, angular velocities corresponding to pitch, roll, and yaw, and the motor speed in rpm of all four motors.The twelve control inputs for the simulation are all of these same values except for the motor speeds, \textcolor{red}{Note - this can likely be referenced from the background} and a simple PID controller uses these states to keep the minimize the error between the flight of the crazyflie and the desired trajectory.
%%% Reference the states actually used by the PID

%% could lead into discussion of the requirements to run on physical experiments, but likely that is best saved for a separate section or the appendix, so this discussion can be referenced





==> Notes_Questions/CR_Exp_Set.tex <==
\section{Experimental Setup}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Overview}
The simulated testing of satellite trajectories proceeds in this implementation as follows. First, the trajectory is calculated, then it is scaled down to an appropriate size to be flown on a crazyflie 2.x and fit into waypoints that the crazyflie can follow. Then a flight simulation is run wherein the desired waypoints are fed to the crazyflie, and the crazyflie's state is observed during this simulated flight for the use of a simple PID controller. This general structure is illustrated in the workflow block diagram in figure [].

\begin{figure}[hbt!]
    \centering
    \includegraphics[width = .49\textwidth]{Figures/WPBlockDiagram.png}
    \caption{Workflow Block Diagram}
    \label{fig:WPBlockDiagram}
\end{figure}

\subsection{Trajectory Creation}
There are multiple implementations to the creation of the satellite trajectory, all of which calculate the linearized hill's equations discussed in background of this paper. The implementations differ in whether hill's equations are in their continuous or discrete expression. Both have fully implemented the A and B matrices which handle current state of and current control inputs of the satellite, respectively. The control inputs are all set to be zero for natural motion trajectories, but the inclusion of these control forces allows for the testing of controlled satellite trajectories, which is the natural progression of terrestrial satellite testing and is likely to be of much higher interest moving forward. 


\subsection{Waypoint Creation}
After the trajectory is made, it must be scaled for use with the crazyflies and then fit into waypoints to be communicated to the crazyflie. The distance is scaled by dividing the x, y, and z components by a common scalar. The format to express the trajectory can be understood by examining the communication between the crazyflie drone and any script it works with. As explained \hl{in the background}, this communication is done at a frequency of 48 Hz for the control of the drone in simulation []. It is then necessary for any trajectory to be fit into waypoints updated at this frequency. This is where the major differences between implementations arise. Both implementations iteratively solve the trajectory, the continuous case using a solver with a set step size and the discrete case naturally falling into the correct format without the error introduced by using a solver.

\subsection{Simulation Flight}
Now that the trajectories have been calculated, scaled, and formatted correctly, the remaining step is for this trajectory to be fed to the crazyflie and its flight following this trajectory is simulated. Within the scope of this paper, it is worth briefly detailing the observation and control of the crazyflie within the gym environment. An observation vector is made for each step of the gym environment with a smaller control vector* using these observed state, as described in the background. A simple PID controller uses these states to minimize the error between the flight of the crazyflie and the desired trajectory, and the simulated flight uses the stepping of the physics, trajectory, and observed state to progress the flight path.

\subsection{Space Dynamics Through Neural Network}
An alternative method of generating a trajectory in the space-scale is through the use of trained three-dimensional simulated neural networks for specific on-orbit scenarios (e.g. docking and inspection) provided by the work in \cite{hamilton2022ablation}. The trajectory outputs of this trained neural networks could be integrated into the existing space-scale to drone-scale conversion architecture as can be seen in Figure \ref{fig:ComBlockDiagram}.

\begin{figure}[htb!]
    \centering
    \includegraphics[width = .49\textwidth]{Figures/CompleteBlockDiagram.png}
    \caption{Workflow Block Diagram with Neural Network}
    \label{fig:ComBlockDiagram}
\end{figure}

==> Notes_Questions/CR_code_implementation.tex <==



The Clohessy-Wiltshire Equations in Hill's frame come in continuous and discrete forms, and toward the interest of creating a more capable and robust testing platform both forms have been implemented. Towards this same end, the structure of this implementation has been carefully made to be robust and scalable with minimal user effort. 


Outline:
Continuous vs discrete - little difference in final result, however because communications with the drones is done on a control frequency, discrete is naturally more fitting for testing because the step size for calculation can be set to perfectly match the control frequency, and calculations can be done without an external solver.

structure:
All variables set in one class - makes adjustments automatic, all matching variables always reference same definition, easy to adjust, adjusts for discrete and continuous at the same time, allows certain variables to be defined by others creating scalability, such as the starting position of the drone being defined as the initial position of the trajectory, so the drone always starts in the correct position. This also makes code more condense and less computationally demanding because the calculation and creation of certain variables/arrays only has to be done once.

From before - the simulation runtime can be set, and then the number of waypoints calculated is automatically fit to fill the full simulation runtime without slowing the trajectory. Trajectory can still be slowed or sped up and fit perfectly to runtime. 

The size of the trajectory is linearly scaled down to run on the drones, x, y, and z are all scaled by the same factor which is adjustable, so the trajectory can be easily scaled to any lab space

Coordinate system - The coordinate system used in creating and communicating the trajectory is a global coordinate system with the origin arbitrarily on the ground. This perfectly matches the coordinate system used by the Lighthouse positioning system in real drones. This means that adjustments necessary for physical testing will be minimal, with the largest difference being the units used for distance are millimeters for the lighthouse system and meters for the simulation, which can be directly addressed by changing the distance scale

The full Clohessy-Wiltshire Equations are implemented, with the control force vector u set to zero for NMT's - this allows for the ability to test/simulate controlled satellite trajectories

Controls:
The trajectory has the structure in place to simulate controlled satellite trajectories for both the discrete and continuous implementations. This means the calculated trajectory can account for control inputs that a satellite would undergo. This trajectory, whether controlled or natural motion, is then scaled down for the drone, and then the drone has its own controller to follow the waypoints of this trajectory. In this implementation, a PID controller is used for the simulated flight, 

%% Probably include as a READ ME in eventual repo

==> Notes_Questions/Literature.tex <==
https://www.youtube.com/@SRCLabCarleton/playlists

Collin:
Read: [1], [2], [3], Onboarding tutorials, its a trap paper

To read: [4], all Potentials, topics under notes


[1] LINCS Simulation Documentation and Overview
[2] Emulation of Close-Proximity Spacecraft Dynamics in Terrestrial Environments Using Unmanned Aerial Vehicles
[3] Model Predictive Control for an Omnidirectional Multi-rotor UAV for Space Applications
[4] Compendium of Relative Motion Concepts in Space
[5] 

Potential:
Wilde, M., Clark, C., and Romano, M., “Historical survey of kinematic and dynamic spacecraft simulators for laboratory
experimentation of on-orbit proximity maneuvers,” Progress in Aerospace Sciences, Vol. 110, 2019, p. 100552.

Pybullet quickstart guide

from LINCS Model Predictive Control for an Omidirectional... paper:

For Hill's frame:
[26] de Ruiter, A., Damaren, C., and Forbes, J., Spacecraft Dynamics and Control: An Introduction, Wiley, 2012.

For Past use of Drones to emulate spacecraft: 
[17] Barari, A., and Ferguson, P., “Dynamic Feasibility of Space Environment Emulation using an Omnidirectional Drone,” 2021
IEEE International Conference on Wireless for Space and Extreme Environments (WiSEE), IEEE, 2021, pp. 66–71.
[18] Barari, A., Dion, R., Jeffrey, I., and Ferguson, P., “Testing satellite control systems with drones,” IEEE Potentials, Vol. 41,
No. 1, 2021, pp. 6–13.
[19] Hamandi, M., Usai, F., Sablé, Q., Staub, N., Tognon, M., and Franchi, A., “Design of multirotor aerial vehicles: A taxonomy
based on input allocation,” The International Journal of Robotics Research, Vol. 40, No. 8-9, 2021, pp. 1015–1044.


References from Arturos Undergrad Thesis:

R. Hewett, S. Puangpontip, “On Controlling Drones for Disaster Relief,” Procedia Computer Science, Volume 207, Pages 3703-3712, 2022

H. M. Sweatland, A. Islay, and W. E. Dixon, “Higher-Order Control Barrier Function for Constraining Position in Motorized Rehabilitative Cycling,” 2021 61st IEEE Conference on Decision and Control (CDC), 2022

K. Dunlap, M. Hibbard, M. Mote, and K. L. Hobbs, “Comparing Run Time Assurance Approaches for Safe Spacecraft Docking,” arXiv:2110.00447v1 [eess.SY], 2021

K. L. Hobbs, M. L. Mote, M. C. L. Abate, S. D. Coogan, and E. M. Feron, “Run Time Assurance for Safety-Critical Systems,” IEEE Control Systems Magazine, Vol 43. No. 2 p. 28-65, 2023

C. I. Chinelato, G. P. Das Neves, and B. A. Angelico, “Safe Control of a Reaction Wheel Pendulum Using Control Barrier Function,” IEEE DOI 10.1109/ACCESS.2020.3018713, 2020

N. Hamilton, K. Dunlap, T. T. Johnson, K. L. Hobbs, “Ablation Study of How Run Time Assurance Impacts the Training and Performance of Reinforcement Learning Agents,” arXiv:2207.04117v1 [cs.LG], 2022

X. Yi, A. Chakarvarthy, and Z. Chen, “Cooperative Collision Avoidance Control of Servo/IPMC Driven Robotic Fish With Back-Relaxation Effect,” IEEE Robotics and Automation Letters, Vol. 6, No. 2, 2021

K. Dunlap, “Run Time Assurance for Intelligent Aerospace Control Systems,” M.S. Thesis submitted to the University of Cincinnati, 2022

K. Zhou, “Safety Control in Quadrotors Based on Control Barrier Function,” M.S. Thesis submitted to Eindhoven University of Technology, 2021

A. D. Ames, S. Coogan, M. Egerstedt, G. Notomista, K, Sreenath, and P. Tabuada, “Control Barrier Functions: Theory and Applications,” arXiv:1903.11100v1 [cs.SY], 2019

A. D. Ames, X. Xu, J. W. Grizzle, and P. Tabuada, “Control Barrier Function Based Quadratic Programs for Safety Critical Systems,” IEEE Transactions and Automatic Control, Vol. 62, No. 8, 2017

C. Luis., J. Le Ny, “Design of a Trajectory Tracking Controller for a Nanoquadcopter,” Mobile Robotics and Autonomous Systems Laboratory, Polytechnique Montreal, 2016

J. Panerati, H. Zheng, S. Zhou, J. Xu, A. Prorok, and A. P. Scheollig, “Learning to Fly – a Gym Environment with PyBullet Physics for Reinforcement Learning of Multi-agent Quadcopter Control,” arXiv:2103.02142v3 [cs.RO], 2021

J. Forster, “System Identification of the Crazyflie 2.0 Nano Quadcopter,” B.S. Thesis submitted to the Institute for Dynamic Systems and Control Swiss Federal Institute of Technology (ETH) Zurich, 2015

P. Wieland and F. Allgöwer, “Constructive safety using control barrier functions,” IFAC Proc. Volumes, vol. 40, no. 12, pp. 462-467, 2007
Himanshu, K. Harikumar, and J. V. Pushpangathan, “Waypoint Navigation of Quadrotor using Deep Reinforcement Learning,” IFAC PapersOnLine 55-22, pgs. 281-286, 2022
A. Taffanel, B. Rousselot, J. Danielsson, K. McGuire, K. Richardsson, M. Eliasson, T. Antonsson, and W. Hönig, “Lighthouse Positioning System: Dataset, Accuracy, and Precision for UAV Research,” arXiv:2104.11523v1 [cs.RO], 2021

==> Notes_Questions/Notes.tex <==
Starting point/references:
Lincs lab
Robitarium
WHAT ARE THE DEMANDS OF THE PEOPLE THAT WILL USE 


We're Distribution A - intended for public release

While Hobbs is out:
Read literature she sent, start on paper
Get gym environment set up on our work computers


People to help with coding problems:
John McCarroll - online only, reach on mattermost
Nate
Safe autonomy chat mattermost
https://www.overleaf.com/project/647df345923d4e8307ee34dc
Collin:
Pg 4 in 
Look into clohessy-wiltshire eqns
what is ray tune
***Confirm whether the crazyflies are 6 degrees of freedom***
Potential - look into kalman filtering


From its a trap prob statement doc:

List of python Libraries requirements - kept in Gitlab, copied out in January 2023 Update presentation
CoRL:https://git.act3-ace.com/act3-rl/corl/-/blob/main/pyproject.toml
Safe Autonomy Sims: https://git.act3-ace.com/rta/safe-autonomy-stack/safe-autonomy-sims/-/blob/main/requirements.txt
Run Time Assurance: 
https://git.act3-ace.com/rta/safe-autonomy-stack/run-time-assurance/-/blob/main/requirements.txt
Safe Autonomy Dynamics: https://git.act3-ace.com/rta/safe-autonomy-stack/safe-autonomy-dynamics/-/blob/main/requirements.txt 



From ITS A TRAP document:

Publications in peer-reviewed journals

		***** Articles beyond this point were pre-work towards the SDCP ***** 
Kyle Dunlap, Mark Mote, Kaiden Delsing, Christopher W. Hays, Kerianne L. Hobbs, “Safe Satellite Docking via Run Time Assured Reinforcement Learning” AIAA Journal of Aerospace Information Systems. 31 Oct 2022
Kyle Dunlap, Michael Hibbard, Mark Mote, and Kerianne Hobbs “Comparing Run Time Assurance Approaches for Safe Spacecraft Docking,” IEEE Control Systems Letters (L-CSS), 2021. Preprint: https://arxiv.org/pdf/2110.00447  

Magazine Articles

		***** Articles beyond this point were pre-work towards the SDCP ***** 
Kerianne L. Hobbs, Mark L. Mote, Matthew C.L. Abate, Samuel D.  Coogan, and Eric M. Feron “Run Time Assurance for Safety Critical Systems: An Introduction to Safety Filtering Approaches for Complex Control Systems,” IEEE Control Systems Magazine, April 2023. Preprint  https://arxiv.org/pdf/2110.03506.pdf 

Technical Papers 

[Draft] Joseph B. Lyons, Kerianne Hobbs, Steve “Cap” Rogers, Scott H. Clouse, “Responsible (Use of) AI,” in Understanding the Role of Humanity in Responsible Deployment of Intelligent Technologies in Socio-technical Ecosystems, Special Issue of Frontiers in Neuroergonomics, 2023.
[In Draft] Kerianne Hobbs, Bernard Li, “Safety, Trust, and Ethics Considerations for Human-AI Teaming in Aerospace Control,” AIAA SciTech,8–12 January 2024, Orlando, FL.
[Submitted] Kyle Dunlap, David Van Wijk, and Kerianne Hobbs, "Run Time Assurance for Autonomous Spacecraft Inspection" 2023 AAS/AIAA Astrodynamics Specialist Conference, Big Sky, MT, August 13-17, 2023 Preprint: https://arxiv.org/pdf/2302.02885  
[Submitted] Nathaniel Hamilton, Kyle Dunlap, Taylor T Johnson, Kerianne Hobbs, “Ablation Study of How Run Time Assurance Impacts the Training and Performance of Reinforcement Learning Agents,” IEEE Space Mission Challenges for Information Technology - IEEE Space Computing Conference, Caltech, Pasadena, CA, USA - 18-21 July 2023. Preprint: https://arxiv.org/pdf/2207.04117 
[Accepted] Umberto Ravaioli, Kyle Dunlap, and Kerianne Hobbs “A Universal Framework for Generalized Run Time Assurance with JAX Automatic Differentiation” American Control Conference, May 31-June 2, 2023, San Diego, CA. Preprint: https://arxiv.org/pdf/2209.01120 
Kerianne L. Hobbs, Joseph B. Lyons, Martin S. Feather, Benjamin P Bycroft, Sean Phillips, Michelle Simon, Mark Harter, Kenneth Costello, Philip C. Slingerland, Yuri Gawdiak, Stephen Paine, “Space Trusted Autonomy Readiness Levels,” IEEE Aerospace, Big Sky, MT, March 4-11, 2023. Preprint: https://arxiv.org/pdf/2210.09059 
                	***** Articles beyond this point were pre-work towards the SDCP *****      
Michael Hibbard, Ufuk Topcu, and Kerianne Hobbs, “Guaranteeing  Safety via Active Set Invariance Filters for Multi-agent Space Systems with Coupled Dynamics,” IEEE American Control Conference, June 8-10, 2022
Kyle Dunlap, Michael Hibbard, Mark Mote, and Kerianne Hobbs “Comparing Run Time Assurance Approaches for Safe Spacecraft Docking,” IEEE American Control Conference, June 8-10, 2022. Preprint: https://arxiv.org/pdf/2110.00447 
Umberto Ravaioli, James Cunningham, John McCarroll, Vardaan Gangal, Kyle Dunlap, and Kerianne Hobbs, “Safe Reinforcement Learning Benchmark Environments for Aerospace Control Systems” IEEE Aerospace Conference, March 2022, Big Sky, MT.
Preston K. Robinette, Benjamin K. Heiner, Umberto Ravaioli, Nathaniel Hamilton, Taylor Johnson, and Kerianne L. Hobbs, “Reinforcement Learning Heuristics for Aerospace Control Systems” IEEE Aerospace Conference, March 2022, Big Sky, MT.
Kyle Dunlap, Mark Mote, Kaiden Delsing, Kerianne L. Hobbs, “Safe Satellite Docking via Run Time Assured Reinforcement Learning” AIAA SciTech, San Diego, CA 2022.
Kyle Dunlap, Kelly Cohen, and Kerianne Hobbs, “Comparing the Explainability and Performance of Reinforcement Learning and Genetic Fuzzy Systems for Safe Satellite Docking,” North American Fuzzy Information processing Society NAFIPS’2021, Virtual, June 7-9, 2021. Outstanding Paper Award
Christopher D. Petersen, Sean Phillips, Kerianne L. Hobbs, and Kendra Lang, “Challenge Problem: Assured Satellite Proximity Operations” 1st AAS/AIAA Space Flight Mechanics Meeting, Virtual, February 1-4, 2021.
Mark Mote, Chris W. Hays, Alexander R. Collins, Eric M. Feron, Kerianne L. Hobbs “Natural Motion-based Trajectories for Automatic Spacecraft Collision Avoidance During Proximity Operations,” IEEE Aerospace, Big Sky, MT, 6-13 Mar 2021.
Kerianne L. Hobbs, Jennifer Davis, Lucas Wagner, and Eric M Feron, “Formal Specification and Analysis of Spacecraft Collision Avoidance Run Time Assurance Requirements.” IEEE Aerospace, Big Sky, MT, 6-13 Mar 2021, Best Paper Award of 35 papers in track.
Kerianne L. Hobbs, Alexander R. Collins, and Eric Feron, “Risk-Based Formal Requirement Elicitation for Automatic Spacecraft Maneuvering,” AIAA SciTech, 11-15 Jan 2021, Nashville, TN.


    \item change time scales (make scalable in one place in the code for easy transition to other labs)
    \item change distance scales (make scalable in one place in the code for easy transition to other labs)
    \item define how space reference frame (CWH) 
    \item define constraints and limitations
    \begin{itemize}
        \item mathematically define geofence for the lab (max range of the drones in the cage
        \item mathematically define constraints for the vehicles relative to each other, e.g. max distance above/below vs. side to side
    \end{itemize}
\end{itemize}

\begin{table}
\renewcommand{\arraystretch}{1.3}
\caption{\bf Summary of Due Dates}
\label{DueDates}
\centering
\begin{tabular}{|c|c|}
\hline
\bfseries Event & \bfseries Due Date \\
\hline\hline
Abstracts Due               & July 1, 2023 \\
Draft Paper {\bf Deadline} & October 6, 2023 \\
Revised papers Due          & January 12, 2024\\
IEEE Copyright Form Due     & January 12, 2024\\
\hline
\end{tabular}
\end{table}

\begin{equation}
{\bf F}=m{\bf a}
\end{equation}
\begin{equation}
e=mc^2
\end{equation}

==> Sections/4_Experimental_Setup.tex <==
\subsection{Overview}
The general process of converting space dynamics to the terrestrial Crazyflie surrogates in simulation is as follows. First, the trajectory of the spacecraft under CW dynamics is calculated. Second, the spacecraft trajectory is scaled to an appropriate size to be flown on a Crazyflie 2.1 and duration is shortened to represent the entire path well within the battery life of the Crazyflie, and then converted into waypoints that the Crazyflie can follow. Third, Crazyflie tracking commands are generated using a PID controller\cite{mellinger2011minimum}. Fourth, a Crazyflie flight following these waypoints is simulated using the PID control commands. Figure \ref{fig:WPBlockDiagram} shows a simplified block diagram of this complete process.

%\subsection{Overview}
%There are two main avenues with which spacecraft dynamics are tested in this work fall under: CWH tests and neural network tests. In the former, natural motion and controlled spacecraft trajectories governed by the linearized Clohessy-Wiltshire equations in Hill's frame are calculated, formatted, and flown on Crazyflies, and in the latter docking scenarios controlled by a reinforcement learning agent are tested.
%Note - can become three avenues if swarms are added to the paper, and four if we include physical testing
%Note - the workflow diagram was made for specifically testing the CWH equations, and not for testing RL agent controlled flight, so the workflow better serves to introduce the CWH section rather than as an overview for both if both are not described by it.

\begin{figure}[hbt!]
    \centering
    \includegraphics[width = .49\textwidth]{Figures/WPBlockDiagram.png}
    \caption{Workflow Block Diagram}
    \label{fig:WPBlockDiagram}
\end{figure}

\subsection{Space Dynamics Simulator}
Before being simulated on the Crazyflie surrogate, a spacecraft's motion in the space-scale Hill's frame is determined. This has been accomplished for both the continuous and discrete representations of the equations, but for convenience only the continuous form will be explained. The simplest Hill's frame trajectory, the NMT introduced in Equation \ref{eqn: CWEquation}, was solved using a Runge-Kutta 45 solver. Note that the output is formatted such that the orbital period and simulation runtime are adjustable independently from each other. The spacecraft dynamics simulators were created as waypoint generating classes which convert the space-scale outputs of the Clohessy-Wiltshire solutions to the drone-scale and seamlessly integrates into the existing trajectory input tools available in \texttt{gym-pybullet-drones}. 
\subsection{Waypoint Generation}
Depending on the time span and the solver step size chosen, the simulator generates a number of waypoints for the simulated drone to follow. 
 Before the waypoints are sent to the simulator, the distance is scaled from the space-scale to the lab-scale, where the lab space is assumed to not be any larger than 4x3x2.5 meters. The distance scale is a factor of 4e3. The waypoints generated serve as discrete position inputs for the drone simulation system, where the amount of waypoints solved correlates to the control frequency multiplied by the chosen time period. Figure \ref{fig:NMTTrajectory} shows an example of the waypoints generated for an in-plane NMT where both the chief and the target remain in the same relative orbital plane (the z-axis, in this and future examples).
 \begin{figure}[htb!]
    \centering
    \includegraphics[width = .49\textwidth]{Figures/NMTTrajectory.png}
    \caption{Lab-Scale, In-Plane Natural Motion Trajectory}
    \label{fig:NMTTrajectory}
\end{figure}
The type of trajectory generated by the Clohessey-Wiltshire equations are dependent on the initial states (three position and three velocity components) of the system. The initial conditions used in this example are as follows (note distances are in meters and velocities are in meters per second),
\begin{equation}
    \centering
    \begin{matrix}
        x =  800  & \dot{x} = 0.16 \\
        \\
        y = \frac{2\dot{x}}{n} & \dot{y} = -2nx \\
        \\
        z = 0 & \dot{z} = 0\\
    \end{matrix}
    \label{eqn: ICs}
\end{equation}
These initial conditions were arbitrarily chosen to loosely model in-space/on-orbit servicing, assembly, and manufacturing (OSAM/ISAM) servicing between two bodies \cite{arney2021orbit}. This simplified simulator was used to generate NMTs and completely makes up the 'Spacecraft Dynamics' block in Figure \ref{fig:WPBlockDiagram}.

 \subsection{Tracking Commands}
 The drone's initial position is chosen to equal the lab-scale initial positions in the space dynamics simulator with the starting rotational position being,
\begin{equation}
\theta_0 = \
    \begin{bmatrix}
        0\\
        0\\
        \pi/2\\
    \end{bmatrix}
\end{equation}
relative to the origin. This initial rotational position starts the drone with all four propellers facing upwards. The simulated drone acts as the deputy spacecraft surrogate and the origin of the inertially fixed frame as the chief. The generated waypoints are then injected into the flight simulator where the drone is controlled by the PID controller introduced in Section 2. 
 
\subsection{Space Dynamics Through Neural Network}
An alternative method of generating a trajectory in the space-scale is through the use of trained three-dimensional simulated neural networks for specific on-orbit scenarios (e.g. docking and inspection) provided by the work in \cite{hamilton2022ablation}. In this implementation, the trained neural network outputs control thrusts to the linearized Clohessy-Wiltshire equations which outputs trajectory data to be integrated into the existing space-scale to drone-scale conversion architecture as can be seen in Figure \ref{fig:ComBlockDiagram}.

%CR - There are two implementations for testing. The first is just reading a saved output, formatting it, and flying it. this allows for testing the RL agent, but in a trivial and non robust way.
%The second uses a saved checkpoint of the RL agent to calculate the trajectory which is then directly formatted and flown. This allows one to easily show that the RL agent is capable of docking from different initial positions/conditions, because the initial conditions are randomly chosen every time the RL agent runs.

\begin{figure}[htb!]
    \centering
    \includegraphics[width = .49\textwidth]{Figures/CompleteBlockDiagram.png}
    \caption{Workflow Block Diagram with Neural Network}
    \label{fig:ComBlockDiagram}
\end{figure}
